Distantly Supervised Transformers For E-Commerce Product QA

We propose a practical instant question answering (QA) system on product pages of ecommerce services, where for each user query, relevant community question answer (CQA) pairs are retrieved. User queries and CQA pairs differ significantly in language characteristics making relevance learning difficult. Our proposed transformer-based model learns a robust relevance function by jointly learning unified syntactic and semantic representations without the need for human labeled data. This is achieved by distantly supervising our model by distilling from predictions of a syntactic matching system on user queries and simultaneously training with CQA pairs. Training with CQA pairs helps our model learning semantic QA relevance and distant supervision enables learning of syntactic features as well as the nuances of user querying language. Additionally, our model encodes queries and candidate responses independently allowing offline candidate embedding generation thereby minimizing the need for real-time transformer model execution. Consequently, our framework is able to scale to large e-commerce QA traffic. Extensive evaluation on user queries shows that our framework significantly outperforms both syntactic and semantic baselines in offline as well as large scale online A/B setups of a popular e-commerce service.

==> expt_qualitative.tex <==
\begin{table*}[h]
\begin{tabular}{lll}
\parbox[t]{3.5cm}{User query} & \parbox[t]{5.5cm}{Top CQA pair retrieved by SemQA-CQA-DS} & \parbox[t]{5.5cm}{Top CQA pair retrieved by E-commerce Baseline} \\ \hline
\multicolumn{3}{c}{Improving semantic relevance} \\ \hline
\parbox[t]{3.5cm}{Do you have size variation??? Like i need  this in bigger wood..} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Is this available in still large size \\ \textbf{A:} yes .. available size is 7*5,8*6,9*7,12*9 in inches} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Is the wood and print waterproof ? \\ \textbf{A:} YES} \\
\parbox[t]{3.5cm}{It is compatible in gaming} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Does it  run gta v \\ \textbf{A:} Yesss... Very fine} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Is it compatible with Amd A6 processor ? \\ \textbf{A:} Yes it's compatible DDR4} \\
\parbox[t]{3.5cm}{Total weight} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Each 1 how to kgs \\ \textbf{A:} 10 kgs} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Total diameter of the plates? \\ \textbf{A:} Plate Dia is 9.5 inches Hole Dia is 30 mm} \\ [0.75cm] \hline
\multicolumn{3}{c}{Improving coverage} \\ \hline 
\parbox[t]{3.5cm}{What is fabric} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Which material is the scarf made up of \\ \textbf{A:} It is like soft satin silk} & 
    \parbox[t]{5.5cm}{No response} \\
\parbox[t]{3.5cm}{The dress with hands or seelveless} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Is it sleeveless \\ \textbf{A:} we give a extra sleeves so u can attach or not..as ur wish} & 
    \parbox[t]{5.5cm}{No response} \\
\parbox[t]{3.5cm}{Bettry perfon} & 
    \parbox[t]{5.5cm}{\textbf{Q:} Batrrey capictiy \\ \textbf{A:} This Phone has a Wonderful 4000 Mah Battery with Battery Saver Options \& Can Watch videos continuously for 18 Hours!!!} & 
    \parbox[t]{5.5cm}{No response} \\ \hline
\end{tabular}
\caption{Qualitative examples.}
\label{table:qualitative-results}
\end{table*}
